Imperfect Knowledge in Autonomous Urban Traffic Manoeuvres

Urban Multi-lane Spatial Logic (UMLSL) was introduced in [13] for proving safety (collision freedom) in autonomous urban traffic manoeuvres with perfect knowledge. We now consider a concept of imperfect knowledge, where cars have less information about other cars. To this end, we introduce the concept of a multi-view and propose crossing controllers using broadcast communication with data constraints for turning manoeuvres at intersections.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{L. Bulwahn, M. Kamali, S. Linker (Eds.): First Workshop on\\ Formal Verification of Autonomous Vehicles (FVAV 2017).\\
EPTCS 257, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.257.7}{10.4204/EPTCS.257.7}}
\pdfoutput=1

